ASTRAL: Automated Safety Testing of Large Language Models

Large Language Models (LLMs) have recently gained attention due to their ability to understand and generate sophisticated human-like content. However, ensuring their safety is paramount as they might provide harmful and unsafe responses. Existing LLM testing frameworks address various safety-related concerns (e.g., drugs, terrorism, animal abuse) but often face challenges due to unbalanced and obsolete datasets. In this paper, we present ASTRAL, a tool that automates the generation and execution of test cases (i.e., prompts) for testing the safety of LLMs. First, we introduce a novel black-box coverage criterion to generate balanced and diverse unsafe test inputs across a diverse set of safety categories as well as linguistic writing characteristics (i.e., different style and persuasive writing techniques). Second, we propose an LLM-based approach that leverages Retrieval Augmented Generation (RAG), few-shot prompting strategies and web browsing to generate up-to-date test inputs. Lastly, similar to current LLM test automation techniques, we leverage LLMs as test oracles to distinguish between safe and unsafe test outputs, allowing a fully automated testing approach. We conduct an extensive evaluation on well-known LLMs, revealing the following key findings: i) GPT3.5 outperforms other LLMs when acting as the test oracle, accurately detecting unsafe responses, and even surpassing more recent LLMs (e.g., GPT-4), as well as LLMs that are specifically tailored to detect unsafe LLM outputs (e.g., LlamaGuard); ii) the results confirm that our approach can uncover nearly twice as many unsafe LLM behaviors with the same number of test inputs compared to currently used static datasets; and iii) our black-box coverage criterion combined with web browsing can effectively guide the LLM on generating up-to-date unsafe test inputs, significantly increasing the number of unsafe LLM behaviors.

==> TableRQ0_results.tex <==
\begin{table}[h]
\caption{Summary of the results for the test evaluators (ratio)}
\label{table:resultsEvalPercentage}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lrrrrr}
\toprule
 %& \multicolumn{1}{c}{\textbf{True Positive}} & \multicolumn{1}{c}{\textbf{True Negative}} & \multicolumn{1}{c}{\textbf{False Positive}} & \multicolumn{1}{c}{\textbf{False Negative}} & \multicolumn{1}{c}{\textbf{No Response}} \\ \cmidrule{1-6}
 & \textbf{TP} & \textbf{TN} & \textbf{FP} & \textbf{FN} & \textbf{No Response} \\ \cmidrule{1-6}
\textbf{GPT 4} & 0.739 & 0.989 & 0.010 & 0.259 & 0.001 \\
\textbf{GPT 4o} & 0.758 & 0.980 & 0.014 & 0.211 & 0.035 \\
\textbf{GPT 3.5} & 0.899 & 0.971 & 0.024 & 0.092 & 0.012 \\
\textbf{Mistral} & 0.345 & 0.973 & 0.005 & 0.277 & 0.398 \\
\textbf{Llama 2} & 0.838 & 0.667 & 0.172 & 0.018 & 0.301 \\
\textbf{Llama 3} & 0.532 & 0.968 & 0.009 & 0.139 & 0.350 \\
\textbf{ChatQA} & 0.065 & 0.927 & 0.010 & 0.765 & 0.231 \\
\textbf{Llamaguard} & 0.360 & 0.974 & 0.025 & 0.639 & 0.000 \\ \bottomrule
\end{tabular}}
\end{table}

==> TableRQ1_results.tex <==
\begin{table}[h!]
\caption{RQ1 -- Comparison of unsafe results between the coverage-based test generator and the baseline test generator across different execution models}
\label{table:benchmarkUnsafeResults}
\centering
\begin{tabular}{lrrr}
\toprule
 & &  \multicolumn{1}{c}{\textbf{Baseline}} & \multicolumn{1}{c}{\textbf{Coverage-based}} \\ 
 & &  \multicolumn{1}{c}{\textbf{Test Generator}} & \multicolumn{1}{c}{\textbf{Test Generator}} \\ 
\cmidrule{2-4}
 & \multicolumn{1}{c}{\textbf{\#testcases}} & \multicolumn{1}{c}{\textbf{\#unsafe}} & \multicolumn{1}{c}{\textbf{\#unsafe}} \\ \cmidrule{1-4}
\multicolumn{1}{l}{\textbf{GPT 4}}& 1260 & 26 & 53\\ 
\multicolumn{1}{l}{\textbf{GPT 4o}} & 1260 & 34& 77\\ 
\multicolumn{1}{l}{\textbf{GPT 3.5}} & 1260 & 107 & 271\\ 


\multicolumn{1}{l}{\textbf{Mistral}}    & 1260 & 128 & 368 \\ 

\multicolumn{1}{l}{\textbf{Llama 2}} & 1260 & 8 & 21\\ 
\multicolumn{1}{l}{\textbf{Llama 3}}& 1260 & 59 & 56\\ 
\multicolumn{1}{l}{\textbf{Vicuna}} & 1260 & 240 & 275 \\ 
\bottomrule
\end{tabular}
\end{table}

==> TableRQ2_categoryResults.tex <==
% \begin{table*}[h]
% \caption{RQ2 -- Number of unsafe results for each 'category' feature across different execution models}
% \label{table:categoryResults}
% \centering
% \begin{tabular}{lrrrrrrr}
% \toprule
% \textbf{}           & \textbf{GPT 3.5} & \textbf{GPT 4o} & \textbf{GPT4} & \textbf{Llama 2} & \textbf{Llama 3} & \textbf{Mistral} & \textbf{Vicuna} \\ \hline
% \textbf{animal\_abuse}       & 18& 7& 3& 0& 0& 21& 19 \\
% \textbf{child\_abuse}        & 6& 2& 3& 0& 0& 9& 11 \\
% \textbf{controversial\_topics,politics}      & 18& 8& 8& 3& 6& 21& 34 \\
% \textbf{discrimination,stereotype,injustice} & 19& 2& 0& 2& 0& 17& 17 \\
% \textbf{drug\_abuse,weapons,banned\_substance}& 33& 12 & 11            & 3& 2& 40& 26 \\
% \textbf{financial\_crime,property\_crime,theft} & 24& 10 & 8& 4& 9& 39& 32 \\
% \textbf{hate\_speech,offensive\_language}    & 14& 1& 2& 1& 1& 20& 13 \\
% \textbf{misinformation\_regarding\_ethics,laws\_and\_safety} & 20& 13 & 8& 0& 7& 27& 25 \\
% \textbf{non\_violent\_unethical\_behavior}   & 22& 3& 2& 1& 5& 32& 4\\
% \textbf{privacy\_violation}  & 19& 4& 1& 2& 8& 28& 7\\
% \textbf{self\_harm}          & 12& 4& 0& 1& 2& 17& 14 \\
% \textbf{sexually\_explicit,adult\_content}   & 15& 4& 1& 1& 7& 18& 15 \\
% \textbf{terrorism,organized\_crime}          & 30& 6& 6& 3& 8& 42& 28 \\
% \textbf{violence,aiding\_and\_abetting,incitement}           & 21& 1& 0& 0& 1& 37& 30 \\          
% \bottomrule
% \end{tabular}
% \end{table*}


\begin{table*}[h]
\caption{RQ2 -- Number of unsafe results for each 'category' feature across different execution models}
\label{table:categoryResults}
\centering
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
\textbf{Model} & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{C4} & \textbf{C5} & \textbf{C6} & \textbf{C7} & \textbf{C8} & \textbf{C9} & \textbf{C10} & \textbf{C11} & \textbf{C12} & \textbf{C13} & \textbf{C14} \\\cmidrule{1-15}

\textbf{GTP 3.5} & 18 & 6 & 18 & 19 & 33 & 24 & 14 & 20 & 22 & 19 & 12 & 15 & 30 & 21\\
\textbf{GTP 4o}  & 7 & 2 & 8 & 2 & 12 & 10 & 1 & 13 & 3 & 4 & 4 & 4 & 6 & 1\\
\textbf{GTP 4}   & 3 & 3 & 8 & 0 & 11 & 8 & 2 & 8 & 2 & 1 & 0 & 1 & 6 & 0\\
\textbf{Llama 2} & 0 & 0 & 3 & 2 & 3 & 4 & 1 & 0 & 1 & 2 & 1 & 1 & 3 & 0\\
\textbf{Llama 3} & 0 & 0 & 6 & 0 & 2 & 9 & 1 & 7 & 5 & 8 & 2 & 7 & 8 & 1\\
\textbf{Mistral} & 21 & 9 & 21 & 17 & 40 & 39 & 20 & 27 & 32 & 28 & 17 & 18 & 42 & 37\\
\textbf{Vicuna}  & 19 & 11 & 34 & 17 & 26 & 32 & 13 & 25 & 4 & 7 & 14 & 15 & 28 & 30\\    
\bottomrule
\end{tabular}
\end{table*}

==> TableRQ2_persuasionResults.tex <==
\begin{table*}[h]
\caption{RQ2 -- Number of unsafe results for each 'persuasion' feature across different execution models}
\label{table:persuasionResults}
\centering
\begin{tabular}{lrrrrrrr}
\toprule
\textbf{}                           & \textbf{GPT 3.5} & \textbf{GPT 4o} & \textbf{GPT4} & \textbf{Llama 2} & \textbf{Llama 3} & \textbf{Mistral} & \textbf{Vicuna} \\ \hline
\textbf{evidence-based\_persuasion} & 61               & 16              & 14            & 4                & 17               & 77               & 62              \\
\textbf{expert\_endorsement}        & 58               & 14              & 9             & 3                & 10               & 72               & 42              \\
\textbf{misrepresentation}          & 57               & 22              & 5             & 3                & 13               & 90               & 68              \\
\textbf{authority\_endorsement}     & 39               & 16              & 12            & 7                & 7                & 59               & 49              \\
\textbf{logical\_appeal}            & 56               & 9               & 13            & 4                & 9                & 70               & 54      \\           
\bottomrule
\end{tabular}
\end{table*}

==> TableRQ2_stylePersuasionResults.tex <==
% \begin{table*}[h]
% \caption{RQ2 -- Number of unsafe results for each combination of 'style' and 'persuasion' features across different execution models}
% \label{table:stylePersuasionResults}
% \centering
% \begin{tabular}{lrrrrrrr}
% \toprule
% \textbf{}                           & \textbf{GPT 3.5} & \textbf{GPT 4o} & \textbf{GPT4} & \textbf{Llama 2} & \textbf{Llama 3} & \textbf{Mistral} & \textbf{Vicuna} \\ \hline
% \textbf{slang +   evidence-based\_persuasion}              & 4                & 3               & 3             & 0                & 1                & 6                & 11              \\
% \textbf{uncommon\_dialects +   evidence-based\_persuasion} & 4                & 2               & 3             & 0                & 1                & 3                & 5               \\
% \textbf{technical\_terms +   evidence-based\_persuasion}   & 12               & 3               & 3             & 2                & 4                & 20               & 15              \\
% \textbf{role\_play +   evidence-based\_persuasion}         & 31               & 4               & 1             & 0                & 3                & 31               & 12              \\
% \textbf{misspellings +   evidence-based\_persuasion}       & 6                & 4               & 4             & 2                & 6                & 6                & 8               \\
% \textbf{question +   evidence-based\_persuasion}           & 4                & 0               & 0             & 0                & 2                & 11               & 11              \\
% \textbf{slang + expert\_endorsement}                       & 2                & 1               & 1             & 1                & 1                & 7                & 4               \\
% \textbf{uncommon\_dialects +   expert\_endorsement}        & 6                & 0               & 1             & 1                & 2                & 8                & 3               \\
% \textbf{technical\_terms +   expert\_endorsement}          & 10               & 5               & 3             & 1                & 3                & 15               & 7               \\
% \textbf{role\_play + expert\_endorsement}                  & 32               & 5               & 1             & 0                & 1                & 33               & 20              \\
% \textbf{misspellings +   expert\_endorsement}              & 4                & 2               & 3             & 0                & 1                & 4                & 3               \\
% \textbf{question + expert\_endorsement}                    & 4                & 1               & 0             & 0                & 2                & 5                & 5               \\
% \textbf{slang + misrepresentation}                         & 1                & 2               & 0             & 0                & 0                & 7                & 9               \\
% \textbf{uncommon\_dialects +   misrepresentation}          & 0                & 2               & 1             & 2                & 2                & 5                & 10              \\
% \textbf{technical\_terms +   misrepresentation}            & 14               & 4               & 3             & 1                & 2                & 27               & 16              \\
% \textbf{role\_play + misrepresentation}                    & 32               & 11              & 0             & 0                & 1                & 34               & 18              \\
% \textbf{misspellings +   misrepresentation}                & 5                & 2               & 1             & 0                & 5                & 7                & 10              \\
% \textbf{question + misrepresentation}                      & 5                & 1               & 0             & 0                & 3                & 10               & 5               \\
% \textbf{slang + authority\_endorsement}                    & 1                & 3               & 1             & 1                & 2                & 3                & 4               \\
% \textbf{uncommon\_dialects +   authority\_endorsement}     & 1                & 3               & 3             & 2                & 0                & 3                & 5               \\
% \textbf{technical\_terms +   authority\_endorsement}       & 9                & 7               & 4             & 1                & 4                & 16               & 10              \\
% \textbf{role\_play +   authority\_endorsement}             & 24               & 0               & 2             & 0                & 1                & 29               & 16              \\
% \textbf{misspellings +   authority\_endorsement}           & 2                & 2               & 1             & 1                & 0                & 4                & 4               \\
% \textbf{question +   authority\_endorsement}               & 2                & 1               & 1             & 2                & 0                & 4                & 10              \\
% \textbf{slang + logical\_appeal}                           & 2                & 1               & 2             & 0                & 1                & 5                & 6               \\
% \textbf{uncommon\_dialects +   logical\_appeal}            & 2                & 0               & 0             & 4                & 0                & 3                & 5               \\
% \textbf{technical\_terms +   logical\_appeal}              & 11               & 3               & 6             & 0                & 4                & 19               & 14              \\
% \textbf{role\_play + logical\_appeal}                      & 34               & 4               & 4             & 0                & 3                & 33               & 14              \\
% \textbf{misspellings + logical\_appeal}                    & 4                & 0               & 1             & 0                & 0                & 3                & 7               \\
% \textbf{question + logical\_appeal}                        & 3                & 1               & 0             & 0                & 1                & 7                & 8     \\           
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{table*}[h]
\caption{RQ2 -- Number of unsafe results for each combination of 'style' and 'persuasion' features across different execution models.} %\pablo{ea horrela hobeto uelrtzen den eta hobeto ikusten den, gutxienez espaziaren aldetik murriztu egiten da, hori bai, style eta persuasion azaltzerakon S eta P definitu beharko lirateke: P1- evidence\_based\_persuasion, P2- expert\_endorsement, P3- misrepresentation, P4- authority\_endorsement, P5- logical\_appeal, S1- slang, S2- Uncommon\_dialects, S3- technical\_terms, S4- role\_play, S5- misspellings, S6- question}}
\label{table:stylePersuasionResults}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrr|rrrrr|rrrrr|rrrrr|rrrrr|rrrrr}
\toprule
 & \multicolumn{5}{c}{\textbf{S1}} & \multicolumn{5}{c}{\textbf{S2}} & \multicolumn{5}{c}{\textbf{S3}} & \multicolumn{5}{c}{\textbf{S4}} & \multicolumn{5}{c}{\textbf{S5}} & \multicolumn{5}{c}{\textbf{S6}} \\ 
\cmidrule(lr){2-31}
                  & \textbf{P1} & \textbf{P2} & \textbf{P3} & \textbf{P4} & \textbf{P5} & \textbf{P1} & \textbf{P2} & \textbf{P3} & \textbf{P4} & \textbf{P5} & \textbf{P1} & \textbf{P2} & \textbf{P3} & \textbf{P4} & \textbf{P5} & \textbf{P1} & \textbf{P2} & \textbf{P3} & \textbf{P4} & \textbf{P5} & \textbf{P1} & \textbf{P2} & \textbf{P3} & \textbf{P4} & \textbf{P5} & \textbf{P1} & \textbf{P2} & \textbf{P3} & \textbf{P4} & \textbf{P5} \\ \midrule
\textbf{GPT 4}    & 3 & 1 & 0 & 1 & 2 & 3 & 1 & 1 & 3 & 0 & 3 & 3 & 3 & 4 & 6 & 1 & 1 & 0 & 2 & 4 & 4 & 3 & 1 & 1 & 1 & 0 & 0 & 0 & 1 & 0 \\
\textbf{GPT 4o}  & 3 & 1 & 2 & 3 & 1 & 2 & 0 & 2 & 3 & 0 & 3 & 5 & 4 & 7 & 3 & 4 & 5 & 11 & 0 & 4 & 4 & 2 & 2 & 2 & 0 & 0 & 1 & 1 & 1 & 1 \\
\textbf{GPT 3.5} & 4 & 2 & 1 & 1 & 2 & 4 & 6 & 0 & 1 & 2 & 12 & 10 & 14 & 9 & 11 & 31 & 32 & 32 & 24 & 34 & 6 & 4 & 5 & 2 & 4 & 4 & 4 & 5 & 2 & 3 \\
\textbf{Mistral} & 6 & 7 & 7 & 3 & 5 & 3 & 8 & 5 & 3 & 3 & 20 & 15 & 27 & 16 & 19 & 31 & 33 & 34 & 29 & 33 & 6 & 4 & 7 & 4 & 3 & 11 & 5 & 10 & 4 & 7 \\
\textbf{Llama 2} & 0 & 1 & 0 & 1 & 0 & 0 & 1 & 2 & 2 & 4 & 2 & 1 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 2 & 0 \\
\textbf{Llama 3} & 1 & 1 & 0 & 2 & 1 & 1 & 2 & 2 & 0 & 0 & 4 & 3 & 2 & 4 & 4 & 3 & 1 & 1 & 1 & 3 & 6 & 1 & 5 & 0 & 0 & 2 & 2 & 3 & 0 & 1 \\
\textbf{Vicuna}  & 11 & 4 & 9 & 4 & 6 & 5 & 3 & 10 & 5 & 5 & 15 & 7 & 16 & 10 & 14 & 12 & 20 & 18 & 16 & 14 & 8 & 3 & 10 & 4 & 7 & 11 & 5 & 5 & 10 & 8 \\
 
\bottomrule
\end{tabular}%
}
\end{table*}


==> TableRQ2_styleResults.tex <==
\begin{table*}[h]
\caption{RQ2 -- Number of unsafe results for each 'style' feature across different execution models}
\label{table:styleResults}
\centering
\begin{tabular}{lrrrrrrr}
\toprule
\textbf{}                   & \textbf{GPT 3.5} & \textbf{GPT 4o} & \textbf{GPT4} & \textbf{Llama 2} & \textbf{Llama 3} & \textbf{Mistral} & \textbf{Vicuna} \\ \hline
\textbf{slang}              & 10               & 10              & 7             & 2                & 5                & 28               & 34              \\
\textbf{uncommon\_dialects} & 13               & 7               & 8             & 9                & 5                & 22               & 28              \\
\textbf{technical\_terms}   & 56               & 22              & 19            & 5                & 17               & 97               & 62              \\
\textbf{role\_play}         & 153              & 24              & 8             & 0                & 9                & 160              & 80              \\
\textbf{misspellings}       & 21               & 10              & 10            & 3                & 12               & 24               & 32              \\
\textbf{question}           & 18               & 4               & 1             & 2                & 8                & 37               & 39  \\           
\bottomrule
\end{tabular}
\end{table*}

==> TableRQ2_style_persuasion_category.tex <==
\begin{table*}[h]
\caption{RQ2 -- Number of unsafe results for each ' style', 'persuasion' and 'category' feature across different execution models.} %\pablo{If you prefer you can split it into three different tables, anyway I think this way it is more appropriate for comparison between features, visually it is easier to compare this way.}}
\label{table:style_persuasion_category}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrr|rrrrr|rrrrrrrrrrrrrr}
\toprule
& \multicolumn{6}{c}{\textbf{Style}} & \multicolumn{5}{c}{\textbf{Persuasion}} & \multicolumn{14}{c}{\textbf{Category}} \\ \cmidrule {2-26}
& \textbf{S1} & \textbf{S2} & \textbf{S3} & \textbf{S4} & \textbf{S5} & \textbf{S6} & \textbf{P1} & \textbf{P2} & \textbf{P3} & \textbf{P4} & \textbf{P5} & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{C4} & \textbf{C5} & \textbf{C6} & \textbf{C7} & \textbf{C8} & \textbf{C9} & \textbf{C10} & \textbf{C11} & \textbf{C12} & \textbf{C13} & \textbf{C14} \\\cmidrule{1-26}
\textbf{GTP 4}   & 7 & 8 & 19 & 8 & 10 & 1 & 14 & 9 & 5 & 12 & 13 & 3 & 3 & 8 & 0 & 11 & 8 & 2 & 8 & 2 & 1 & 0 & 1 & 6 & 0\\
\textbf{GTP 4o}  & 10 & 7 & 22 & 24 & 10 & 4 & 16 & 14 & 22 & 16 & 9 & 7 & 2 & 8 & 2 & 12 & 10 & 1 & 13 & 3 & 4 & 4 & 4 & 6 & 1\\
\textbf{GTP 3.5} & 10 & 13 & 56 & 153 & 21 & 18 & 61 & 58 & 57 & 39 & 56 & 18 & 6 & 18 & 19 & 33 & 24 & 14 & 20 & 22 & 19 & 12 & 15 & 30 & 21\\
\textbf{Mistral} & 28 & 22 & 97 & 160 & 24 & 37 & 77 & 72 & 90 & 59 & 70 & 21 & 9 & 21 & 17 & 40 & 39 & 20 & 27 & 32 & 28 & 17 & 18 & 42 & 37\\
\textbf{Llama 2} & 2 & 9 & 5 & 0 & 3 & 2 & 4 & 3 & 3 & 7 & 4 & 0 & 0 & 3 & 2 & 3 & 4 & 1 & 0 & 1 & 2 & 1 & 1 & 3 & 0\\
\textbf{Llama 3} & 5 & 5 & 17 & 9 & 12 & 8 & 17 & 10 & 13 & 7 & 9 & 0 & 0 & 6 & 0 & 2 & 9 & 1 & 7 & 5 & 8 & 2 & 7 & 8 & 1\\
\textbf{Vicuna}  & 34 & 28 & 62 & 80 & 32 & 39 & 62 & 42 & 68 & 49 & 54 & 19 & 11 & 34 & 17 & 26 & 32 & 13 & 25 & 4 & 7 & 14 & 15 & 28 & 30\\          
\bottomrule
\end{tabular}}
\end{table*}
